Robust fine-tuning of zero-shot models

Large pre-trained models such as CLIP or ALIGN offer consistent accuracy across a range of data distributions when performing zero-shot inference (i.e., without fine-tuning on a specific dataset). Although existing fine-tuning methods substantially improve accuracy on a given target distribution, they often reduce robustness to distribution shifts. We address this tension by introducing a simple and effective method for improving robustness while fine-tuning: ensembling the weights of the zero-shot and fine-tuned models (WiSE-FT). Compared to standard fine-tuning, WiSE-FT provides large accuracy improvements under distribution shift, while preserving high accuracy on the target distribution. On ImageNet and five derived distribution shifts, WiSE-FT improves accuracy under distribution shift by 4 to 6 percentage points (pp) over prior work while increasing ImageNet accuracy by 1.6 pp. WiSE-FT achieves similarly large robustness gains (2 to 23 pp) on a diverse set of six further distribution shifts, and accuracy gains of 0.8 to 3.3 pp compared to standard fine-tuning on seven commonly used transfer learning datasets. These improvements come at no additional computational cost during fine-tuning or inference.

==> 01_intro_old.tex <==
\section{Introduction}
\postsec
A foundational goal of machine learning is to develop models that work reliably across a broad range of data distributions. 
ecently, large pre-trained models such as CLIP \cite{radford2021learning} and ALIGN \cite{jia2021scaling} have demonstrated unprecedented robustness to challenging distribution shifts where prior robustness interventions failed to improve performance \cite{taori2020measuring}.
While these results point towards pre-training on large, heterogeneous datasets as a promising direction for increasing robustness, an important caveat is that these robustness improvements occur only in the zero-shot setting, i.e., when the model performs inference without fine-tuning on a specific target distribution \cite{radford2021learning}.


In a concrete application, a zero-shot model can be fine-tuned on extra application-specific data, which often yields large performance gains on the target distribution.
However, Radford \etal \cite{radford2021learning} have shown that current fine-tuning techniques carry a hidden cost: the out-of-distribution accuracy of their fine-tuned CLIP models is often lower than that of the original zero-shot model.
This leads to a natural question: \emph{Can zero-shot models be fine-tuned without reducing out-of-distribution accuracy?}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{new_arxiv_v2/figures/fig1_new.pdf}
    \caption{
    \textbf{(Top left)} Zero-shot CLIP models exhibit high effective robustness and moderate in-distribution accuracy, while standard fine-tuning---either end-to-end or with a linear classifier (final layer)---attains higher ID accuracy and less effective robustness.
    \textbf{(Top right)} Our method linearly interpolates between the zero-shot and fine-tuned models with a mixing coefficient $\alpha \in [0,1]$. \textbf{(Bottom)} On five distribution shifts derived from ImageNet (ImageNetV2, ImageNet-R, ImageNet Sketch, ObjectNet, and ImageNet-A), WiSE-FT improves average OOD accuracy relative to both the zero-shot and fine-tuned models while maintaining or improving ID accuracy.
    }
    \label{fig:fig1}
\end{figure*}

As pre-trained models are becoming a cornerstone of machine learning, techniques for fine-tuning them on downstream applications are increasingly important.
Indeed, the question of robustly fine-tuning pre-trained models has recently also been raised as an open problem by several authors \cite{andreassen2021evolution,bommasani2021opportunities,radford2021learning}. Andreassen \etal \cite{andreassen2021evolution} explored several fine-tuning approaches but found that none yielded models with improved robustness at high accuracy.
Furthermore, Taori \etal \cite{taori2020measuring} demonstrated that no current algorithmic robustness interventions provide consistent gains across the distribution shifts where zero-shot CLIP excels.

In this paper, we conduct an empirical investigation to understand and improve fine-tuning of zero-shot models.
First, we measure how different fine-tuning approaches (last layer vs. end-to-end fine-tuning, hyperparameter changes, etc.) affect the out-of-distribution accuracy of the resulting fine-tuned models.
We find that more aggressive fine-tuning (e.g., using a larger step size) yields larger in-distribution improvements but can also reduce out-of-distribution accuracy by a larger amount.
In addition, out-of-distribution accuracy varies substantially even among models with the same in-distribution accuracy.
Overall, the fine-tuning process is brittle and the best hyperparameters cannot be inferred from in-distribution accuracy alone.

To address these issues, we then introduce a robust way of fine-tuning zero-shot models that achieves the best of both worlds: increased performance out-of-distribution while maintaining or even improving in-distribution accuracy relative to standard fine-tuning. In addition, our method simplifies the choice of hyperparameters in the fine-tuning process.
Our method (Figure \ref{fig:fig1}) has two steps: first, we fine-tune the zero-shot model on application-specific data. Second, we combine the original zero-shot and fine-tuned models by linearly interpolating between their weights, which we refer to as weight-space ensembling. 

Interestingly, linear interpolation in weight space succeeds despite non-linearity in the activation functions of the neural networks.
Weight-space ensembles for fine-tuning (WiSE-FT) substantially improve out-of-distribution accuracy compared to prior work while maintaining high in-distribution performance.
Concretely, on ImageNet \cite{deng2009imagenet} and five of the natural distribution shifts studied by Radford \etal~\cite{radford2021learning}, WiSE-FT applied to standard end-to-end fine-tuning improves out-of-distribution accuracy by 3.9 to 6 percentage points (pp) over prior work while improving the in-distribution accuracy by 1.6 pp.
Relative to the zero-shot model, WiSE-FT improves out-of-distribution accuracy by 1 to 9 pp. Moreover, WiSE-FT improves over a range of alternative approaches such as regularization and evaluating at various points throughout fine-tuning. The robustness comes at no additional computational cost during fine-tuning or inference because the zero-shot and fine-tuned models are ensembled into a single model of the same size.

To understand the robustness gains of WiSE-FT, we empirically analyze ensembling through the lens of distributional robustness. First, we study WiSE-FT when fine-tuning a linear classifier (last layer) as it is amenable to analysis: our procedure is then equivalent to ensembling the outputs of two models, and experiments point towards the complementarity of model predictions as a key property. We illustrate via detailed measurements how the predictions of zero-shot and fine-tuned models are diverse, and that models are more confident on the parts of the test distributions they perform well on.
 \begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{new_arxiv_v2/figures/datasets.pdf}
    \caption{Samples of the class \textit{lemon}, from ImageNet \cite{deng2009imagenet} (in-distribution) and the derived out-of-distribution datasets considered in our main experiments: ImageNet-V2 \cite{pmlr-v97-recht19a}, ImageNet-R \cite{imagenetr}, ImageNet Sketch \cite{imagenetsketch}, ObjectNet \cite{objectnet}, and ImageNet-A \cite{imageneta}.}
    \label{fig:data_samples}
\end{figure*}

For end-to-end fine-tuning, we connect our observations to earlier work on the phenomenology of deep learning. Neyshabur \etal \cite{neyshabur2020being} found that end-to-end fine-tuning the same model twice yielded two different solutions that were connected via a linear path in weight space along which error remains low, known as linear mode connectivity \cite{frankle2020linear}. The authors therefore concluded that the two solutions are in the same basin of the loss landscape. Interestingly, linear interpolation in weight space succeeds despite non-linearity in the activation functions of the neural networks. 
Our observations suggest a similar phenomenon along the path generated by WiSE-FT, but the exact shape of the loss landscape and connection between in- and out-of-distribution error are still an open problem.

In addition to the aforementioned ImageNet distribution shifts, WiSE-FT consistently improves robustness on a diverse set of six further distribution shifts including: (i) geographic shifts in satellite imagery and wildlife recognition (WILDS-FMoW, WILDS-iWildCam) \cite{wilds2021, christie2018functional, beery2021iwildcam}, (ii) reproductions of the popular image classification dataset CIFAR-10 with a distribution shift (CIFAR-10.1 and CIFAR-10.2) \cite{pmlr-v97-recht19a, lu2020harder}, and (iii) datasets with distribution shift induced by temporal perturbations in videos (ImageNet-Vid-Robust and YTBB-Robust) \cite{vidrobust}.



Beyond the robustness perspective, WiSE-FT also improves in-distribution performance compared to standard fine-tuning, reducing the relative error rate by 6 to 62\% on a range of seven datasets: ImageNet, CIFAR-10, CIFAR-100 \cite{krizhevsky2009learning}, Describable Textures \cite{dtd}, Food-101 \cite{food101}, SUN397 \cite{sun397}, and Stanford Cars \cite{cars}.
Even when fine-tuning data is scarce—reflecting many application scenario---we find that WiSE-FT substantially improves in-distribution performance.
When five examples per class are used for fine-tuning, WiSE-FT improves in-distribution performance by 0.3 to 6.1 percentage points compared to the best of the zero-shot and fine-tuned models on the seven aforementioned datasets.
Overall, we find that WiSE-FT is universally applicable in the problems we studied, and we encourage its adoption for fine-tuning zero-shot models.







==> 05_discussion_old.tex <==
\vspace*{-0.1cm}
\beforesec
\section{Discussion}
\label{sec:discussion}
\postsec
This section further analyzes the empirical phenomena we have observed so far.
We begin with the case where only the final linear layer is fine-tuned and predictions from the weight-space ensemble can be factored into the outputs of the zero-shot and fine-tuned model.
Next, we connect our observations regarding end-to-end fine-tuning with earlier work on the phenomenology of deep learning.%
\vspace*{-0.1cm}
\beforesec
\subsection{Zero-shot and fine-tuned models are complementary}
\label{sec:decomposing}
\postsec


In this section, we find that the zero-shot and fine-tuned models have diverse predictions, both on reference and shifted distributions. Moreover, while the fine-tuned models are more confident on the reference distribution, the reverse is true under distribution shift.  

\smallpara{Zero-shot and fine-tuned models are diverse.}
\label{sec:diversity}
In certain cases, ensemble accuracy is correlated with diversity among the constituents \cite{kuncheva2003measures, gontijo2021no}.
If two models make coincident mistakes, so will their ensemble, and no benefit will be gained from combining them. 
Here, we explore two measures of diversity: {\it prediction diversity,} which measures the fraction of examples for which two classifiers disagree but one is correct; and {\it Centered Kernel Alignment Complement,}  the complement of CKA \cite{kornblith2019similarity}. 
Additional diversity measures and details are provided in Appendix \ref{sec:diversity_defs}.
In Figure \ref{fig:diversity_and_confidence} (left), we show that the zero-shot and fine-tuned models are diverse both on the reference and shifted distributions, despite sharing the same backbone. 
As a point of comparison, we include avg. diversity measures between two linear classifiers fine-tuned with random splits on half of 
ImageNet,\footnote{Two linear classifiers fine-tuned on the same data converge to similar solutions, resulting in negligible diversity. 
As a stronger baseline, we fine-tune classifiers on different subsets of ImageNet, with half of the data.} denoted in orange in Figure \ref{fig:diversity_and_confidence}.


\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/diversity_and_confidence.pdf}
    \vspace*{-2.2em}
    \caption{\textbf{(Left)} Zero-shot and fine-tuned models exhibit diversity in their predictions. \textbf{(Middle)} On most distribution shifts, the zero-shot model overrides the linear classifier more than it is overridden. The reverse is true for ImageNet (reference). \textbf{(Right)} Similarly, zero-shot models are more confident under distribution shift, while the reverse is true on the reference distribution. The margin $\delta_f$ measures the average difference between the largest and second largest unormalized output for classifier $f$}
    \vspace*{-1em}
    \label{fig:diversity_and_confidence}
\end{figure*}

\smallpara{Models are more confident where they excel.}
In order for the ensemble model to be effective, it should leverage each model's expertise based on which distribution the data is from.
Here, we empirically show that this occurs on a number of datasets we consider.
First, we examine the cases where the models being ensembled disagree. 
We say the zero-shot model \textit{overrides} the fine-tuned model if their predictions disagree and the zero-shot prediction matches that of the weight-space ensemble. 
Similarly, if models disagree and the linear classifier prediction matches the ensemble, we say the zero-shot is \textit{overridden}.
Figure \ref{fig:diversity_and_confidence} (middle) shows the fraction of samples where the zero-shot model overrides and is overridden by the fine-tuned linear classifier for $\alpha{=}0.5$. 
Other than ImageNetV2, which was collected to closely reproduce ImageNet, the zero-shot model overrides the linear classifier more than it is overridden on the distribution shifts.

Additionally, we are interested in measuring model confidence. Recall that we are ensembling quantities before a softmax is applied, so we avoid criteria that use probability vectors, e.g., \citet{guo2017calibration}.
Instead, we consider the margin $\delta$ between the largest and second largest output of each classifier. 
Figure \ref{fig:diversity_and_confidence} (right) shows that the zero-shot model is more confident in its predictions under distribution shift, while the reverse is true on the reference distribution.
\vspace*{-0.1cm}
\beforesec
\subsection{An error landscape perspective}
\label{sec:landscape}
\postsec
Our discussion now focuses on the empirical phenomenon we observe when weight-space ensembling all layers in the network.
Specifically, this section formalizes our observations and details related phenomena. 
Recall that the weight-space ensemble of $\theta_0$ and $\theta_1$ is given by $f\mleft(x, (1-\alpha)\cdot\theta_0 + \alpha\cdot\theta_1 \mright)$ (Equation~\ref{eqn:wse}).
We begin with a natural generalization of \textit{linear mode connectivity} \cite{frankle2020linear} to the setting where accuracy of the endpoints may differ substantially.
For a distribution $\mathcal{D}$ and model $f$, let $\mathsf{Acc}_{\mathcal{D}, f}(\theta)$ denote the expected accuracy of $f$ evaluated with parameters $\theta$ on distribution $\mathcal{D}$.

\textbf{Definition 1:} Parameters $\theta_0$ and $\theta_1$ exhibit \textit{linear mode connectivity} with respect to $f$ and $\mathcal{D}$ if, for all $\alpha \in [0,1]$, $\mathsf{Acc}_{\mathcal{D}, f}\mleft((1-\alpha)\cdot \theta_0 +  \alpha \cdot \theta_1\mright)\ \geq \ (1-\alpha) \cdot \mathsf{Acc}_{\mathcal{D}, f}\mleft(\theta_0\mright) + \alpha \cdot \mathsf{Acc}_{\mathcal{D}, f}\mleft(\theta_1\mright)$.
Note that when $\mathsf{Acc}_{\mathcal{D}, f}\mleft(\theta_0\mright) = \mathsf{Acc}_{\mathcal{D}, f}\mleft(\theta_1\mright)$, this is equivalent to the original definition \cite{frankle2020linear}.\footnote{The original definition used $\gtrapprox \frac{1}{2}\mleft(\mathsf{Acc}_{\mathcal{D}, f}\mleft(\theta_0\mright) + \mathsf{Acc}_{\mathcal{D}, f}\mleft(\theta_1\mright) \mright)$ and so Definition 1 is not a strict generalization. This original definition is less applicable when endpoint accuracy differs substantially.}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/figure_definition_small.pdf}
    \vspace*{-2em}
    \caption{The zero-shot and fine-tuned models exhibit \textit{linear mode connectivity} \cite{frankle2020linear} on ImageNet and the main distribution shifts we consider (Observation 1). Moreover, there exists an $\alpha$ for which WiSE-FT outperforms both the zero-shot and fine-tuned models (Observation 2).}
    \vspace*{-1.5em}
    \label{fig:def}
\end{figure*}

\textbf{Observation 1:} As illustrated in Figure~\ref{fig:def}, we observe linear mode connectivity on ImageNet and the five associated distribution shifts we consider (Section~\ref{sec:expsetup}).

To assist in contextualizing Observation 1, we review related phenomena. Neural networks are nonlinear, hence weight-space ensembles only achieve good performance in exceptional cases---ensembling two randomly initialized networks in weight-space achieves no better accuracy than a random classifier \cite{frankle2020linear}. 
Linear mode connectivity has been observed by 
\citet{frankle2020linear}; \citet{izmailov2018averaging}  when part of the training trajectory is shared, and by \citet{neyshabur2020being} when two models are fine-tuned with a shared initialization.
In particular, the observations of \citet{neyshabur2020being} may elucidate why weight-space ensembles attain high 
accuracy in the setting we consider, as they suggest that fine-tuning remains in a region where solutions are connected by a linear path along which error remains low.
Instead of considering the weight-space ensemble of two fine-tuned models, we consider the weight-space ensemble of the 
\textit{pre-trained} and fine-tuned models. This is only possible for a pre-trained model capable of zero-shot inference such as CLIP. 


\textbf{Observation 2:} As illustrated by Figure~\ref{fig:def}, on ImageNet and the five associated distribution shifts we consider, weight-space ensembling (end-to-end) may outperform both the zero-shot and fine-tuned models, i.e., there exists an $\alpha$ for which $\mathsf{Acc}_{\mathcal{D}, f}\left((1-\alpha) \cdot \theta_0 +  \alpha \cdot \theta_1\right) \ \geq \ \max\left\{  \mathsf{Acc}_{\mathcal{D}, f}\left(\theta_0\right) ,  \ \mathsf{Acc}_{\mathcal{D}, f}\left(\theta_1\right) \right\}$.

We are not the first to observe that when interpolating between models with linear mode connectivity, the accuracy of models along the path may exceed that of either endpoint \cite{izmailov2018averaging, neyshabur2020being, pmlr-v139-wortsman21a}. \citet{neyshabur2020being}
conjecture that interpolation could produce solutions closer to the true center of a basin. 
In contrast to \citet{neyshabur2020being}, we interpolate between models which observe different data.












==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

